Visual-Oriented Fine-Grained Knowledge Editing for MultiModal Large Language Models

Knowledge editing aims to efficiently and cost-effectively correct inaccuracies and update outdated information. Recently, there has been growing interest in extending knowledge editing from Large Language Models (LLMs) to Multimodal Large Language Models (MLLMs), which integrate both textual and visual information, introducing additional editing complexities. Existing multimodal knowledge editing works primarily focus on text-oriented, coarse-grained scenarios, failing to address the unique challenges posed by multimodal contexts. In this paper, we propose a visual-oriented, fine-grained multimodal knowledge editing task that targets precise editing in images with multiple interacting entities. We introduce the Fine-Grained Visual Knowledge Editing (FGVEdit) benchmark to evaluate this task. Moreover, we propose a Multimodal Scope Classifier-based Knowledge Editor (MSCKE) framework. MSCKE leverages a multimodal scope classifier that integrates both visual and textual information to accurately identify and update knowledge related to specific entities within images. This approach ensures precise editing while preserving irrelevant information, overcoming the limitations of traditional text-only editing methods. Extensive experiments on the FGVEdit benchmark demonstrate that MSCKE outperforms existing methods, showcasing its effectiveness in solving the complex challenges of multimodal knowledge editing.

==> sec/temp-method.tex <==
\begin{figure*}[ht]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[]{pic/method.pdf}

   \caption{Architecture of the FGVEdit method, illustrating the multimodal scope classifier, editing memory, base model with frozen parameters, counterfactual model with trainable parameters, and the decision workflow for handling in-scope and out-of-scope inputs.}
   \label{fig:method}
\end{figure*}

\section{Fine-Grained Visual Knowledge Editing}

\subsection{Problem Formulation}
Fine-grained visual knowledge editing~(FGVEdit) task focuses on updating specific and detailed knowledge within MLLMs that process both visual and textual information. Unlike other multimodal knowledge editing tasks, which treat an image as an entity and perform coarse-grained edits that may overlook complex visual details, FGVEdit aims to modify knowledge related to specific entities and relationships involving multiple interactive elements within complex images.

Formally, let $ f_{\theta} $ denote a pre-trained MLLM with parameters $ \theta $ that can generate outputs based on combined image-text inputs. A sample of the model's editing is represented as $ (i_e, t_e, y_e) $, where $ i_e $ denotes an image containing multiple entities, $ t_e $ is the textual prompt, and $ y_e $ represents the expected output for the input $ (i_e, t_e) $. The model's original output is given by $ y_o = f_{\theta}(i_e, t_e) $ and $y_o \neq y_e$.

The objective of the FGVEdit task is to update the model's knowledge so that it accurately reflects $ y_e $ when queried for specific fine-grained details, without affecting its performance on unrelated content. We define a knowledge editing operation $ \mathcal{E} $ to update the model parameters as $\theta_e = \mathcal{E}(\theta, i_e, t_e, y_e)$.
After applying $\mathcal{E}$, the updated model $ f_{\theta_e} $ should be capable of generating the corrected output for the specific input as $ y_e = f_{\theta_e}(i_e, t_e) $.

\noindent\textbf{Fine-Grained Visual Editing Scope}: For the fine-grained knowledge defined by the editing example $ (i_e, t_e, y_e) $, there exists a fine-grained editing scope $ S(i_e, t_e, y_e) $. This editing scope is determined by both visual and textual information. For in-scope inputs on the same image, represented as $ (i_{e}, t_{in}) \in S(i_e, t_e, y_e) $, the original model's output is $ y_{in} = f_{\theta}(i_e, t_{in}) $, and the edited model is required to produce a correction as $ y\prime_{in} = f_{\theta_e}(i_e, t_{in}) $. For out-of-scope inputs on the same image, represented as $ (i_e, t_{out}) \notin S(i_e, t_e, y_e) $, the original model's output is $ y_{out} = f_{\theta}(i_e, t_{out}) $, and the edited model maintains the original output as $ y_{out} = f_{\theta_e}(i_e, t_{out}) $.

% We consider a pre-trained Multimodal Large Language Model (MLLM), denoted as $f_{\theta}$, where $\theta$ represents the model parameters.
% The input to the model is structured as a pair $(i_e, t_e)$, with $i_e$ indicating the image and $t_e$ representing the corresponding text prompt.
% The original output generated by the model before any editing is denoted as $y_o = f_{\theta}(i_e, t_e)$.
% Let the ground truth output for the input pair $(i_e, t_e)$ be represented as $y_e$, with the condition that $y_o \neq y_e$.

% We define the editing operation applied to the MLLM as a function $\mathcal{E}$, which updates the model parameters based on the provided editing samples. This operation can be expressed mathematically as $\theta_e = \mathcal{E}(i_e, t_e, y_e)$. Consequently, under the modified parameters $\theta_e$, the output of the MLLM is recalibrated to yield $f_{\theta_e}(i_e, t_e) = y_e$.
\subsection{FGVEdit Framework}
Building upon SERAC~\cite{serac}, we propose a Fine-Grained Visual Knowledge Editing (FGVEdit) framework, as illustrated in Fig.~\ref{fig:method}. Structurally, our FGVEdit framework comprises the following four major components: the \textbf{MultiModal Edit Memory}, the \textbf{MultiModal Scope Classifier}, the \textbf{Base MultiModal Model} ($f_{\text{base}}$), and the \textbf{Counterfactual MultiModal Model} ($f_{\text{cfr}}$).

During the editing process, FGVEdit does not modify the model parameters. Instead, it stores the editing examples in the MultiModal Edit Memory. The MultiModal Edit Memory is a model-agnostic component designed to accept and store the knowledge that needs to be updated, represented as edit examples. These examples specify the precise modifications or corrections to the model’s knowledge. By maintaining these edit examples separately, FGVEdit can reference them when necessary without altering the base model directly.

When receiving a new input, the MultiModal Scope Classifier evaluates the relevance of the input to the stored editing examples based on visual and textual information. It then decides whether to invoke the edited information or rely on the base model's response. This ensures that edits are applied appropriately to relevant inputs while unrelated knowledge remains stable. The MultiModal Scope Classifier is defined as $f_{\text{cls}}(i_{\text{test}}, t_{\text{test}}, i_e, t_e, y_e)$.

The index $k^*$ of the most similar editing example and its corresponding similarity $\rho$ are determined as follows:
\begin{align}
k^* &= \mathop{\arg\min}\limits_k f_{\text{cls}}(i_{\text{test}}, t_{\text{test}}, i_e^k, t_e^k, y_e^k), \\
\rho &= f_{\text{cls}}(i_{\text{test}}, t_{\text{test}}, i_e^{k^*}, t_e^{k^*}, y_e^{k^*}),
\end{align}
where $\rho \in [0,1]$. Inputs with similarity less than $0.5$ are considered out-of-scope samples, while those with similarity equal to or greater than $0.5$ are regarded as in-scope samples. The final output of the model is:
\begin{align}
y_{\text{test}} = 
\begin{cases}
f_{\text{base}}(i_{\text{test}}, t_{\text{test}}), & \rho < 0.5, \\
f_{\text{cfr}}(t_e, y_e, i_{\text{test}}, t_{\text{test}}), & \rho \geq 0.5,
\end{cases}
\end{align}
where $f_{\text{base}}$ denotes the base model, and $f_{\text{cfr}}$ denotes the counterfactual model. 

The base multimodal model is the original pretrained multimodal large language model (e.g., MiniGPT-4), designed to process inputs that are unrelated to the editing examples in the multimodal memory. By freezing the parameters of the base multimodal model, we ensure that its general knowledge remains stable and unaffected by the editing examples.
In contrast, the counterfactual multimodal model responds to inputs related to the editing examples. Specifically, the counterfactual multimodal model accepts the input $(i_{\text{test}}, t_{\text{test}})$ while incorporating the corresponding editing examples from the multimodal editing memory. Guided by the prompts of the editing examples in memory, the counterfactual multimodal model generates outputs that reflect the necessary knowledge updates or corrections.
The counterfactual multimodal model can either be a trainable model that shares the same output space as the base multimodal model or employ alternative editing methods that accurately reflect the new facts.
% \subsection{FGVEdit Framework}
% Building upon SERAC\cite{serac}, we propose a fine-grained visual knowledge editing (FGVEdit) framework, as illustrated in Fig.~\ref{fig:method}. Structurally, our FGVEdit framework comprises the following four major components.
% \begin{itemize}
%     \item MultiModal Edit Memory: It is designed to accept and store the knowledge that needs to be updated, represented as edit examples. These examples specify the precise modifications or corrections to the model’s knowledge. By maintaining these edit examples separately, FGVEdit can reference them when necessary without altering the base model directly.
%     \item MultiModal Scope Classifier: It is the crucial component in determining the success of the editing. It evaluates the relevance of the input to the stored edits based on visual and textual information and decides whether to invoke the edited information or rely on the base model's response. This ensures that edits are applied appropriately to relevant inputs while unrelated knowledge remains stable.
%     \item Base MultiModal Model ($f_{\text{base}}$): It is the original pre-trained multimodal large language model (like MiniGPT-4) that serves as the foundation for the knowledge editing process. When the scope classifier determines that an input is unrelated to the stored edit examples, the base model is used to generate responses. By freezing the parameters of the base model during the editing process, we ensure that its general knowledge remains stable and unaffected by the edit examples.
%     \item Counterfactual MultiModal Model ($f_{\text{cfr}}$): It is typically a MLLM with trainable parameters. When the multimodal scope classifier identifies that an input is related to the edit examples, the counterfactual model is used to generate the response. Guided by the prompts from the edit examples in the edit memory, the counterfactual model produces outputs that reflect the desired knowledge updates or corrections. This allows the system to provide accurate and updated responses for inputs that are relevant to the edits.
% \end{itemize}

% \begin{itemize}
%     \item Base MultiModal Model ($f_{\text{base}}$): It's the original pre-trained MultiModal large language model (like MiniGPT-4) that serves as the foundation for the knowledge editing process. 
%     The goal is to retain the vast majority of the original knowledge within this base model while making targeted edits.
%     The parameters of the base model are frozen during the editing process.

%     %The base model remains largely untouched except in specific areas where updates are necessary.
%     \item MultiModal Edit Memory: It is a crucial component that stores and tracks the modifications made to the model. Instead of altering the base model directly, the system maintains a separate memory structure to log edits. This memory allows FGVEdit to efficiently apply knowledge updates without distorting the underlying model’s broader knowledge. The edit memory enables selective recall of the edits, ensuring they are contextually applied only when relevant.
%     \item MultiModal Scope Classifier : It determines the boundaries within which the knowledge edits should apply. This classifier decides whether an input falls within the scope where a specific edit should be activated. By identifying when to use the edited information versus the original base model's knowledge, the scope classifier ensures that the updates do not bleed into unrelated contexts, thus preserving the generalization capabilities of the original model.
%     \item Counterfactual MultiModal Model ($f_{\text{cfr}}$): It is used to generate alternative outputs that simulate how the model should behave after applying the edit. It is a hypothetical model that represents how the base model’s knowledge would change if the new information were integrated. By comparing the outputs of the counterfactual model with the base model, we can assesses the impact of the edits, ensuring that they achieve the intended modifications while minimizing unintended consequences.
% \end{itemize}

%with a Multimodal Classifier~(FGVEdit) method, aiming to address the challenges of fine-grained visual knowledge editing.
%Our method is illustrated in Figure~\ref{fig:method}. FGVEdit primarily relies on a multimodal scope classifier that simultaneously considers image and text information to finely partition the editing scope.

% \subsection{Inference Step}
% The editing step of FGVEdit involves simply storing the edited examples in the multimodal editing memory.
% When we need to use the edited model to infer new input, we first employ the multimodal model classifier to compute the similarity between the input and all edited examples in memory, which is defined as $f_{\text{cls}}(i_{\text{test}}, t_{\text{test}}, i_e, t_e, y_e)$. 
% The index $k^*$ of the most similar editing example and its corresponding similarity $\rho$ can be get as follows:

% \begin{align}
% k^* &= \mathop{\arg\min}\limits_k f_{\text{cls}}(i_{\text{test}}, t_{\text{test}}, i_e^k, t_e^k, y_e^k),
% \\
% \rho &= f_{\text{cls}}(i_{\text{test}}, t_{\text{test}}, i_e^{k^*}, t_e^{k^*}, y_e^{k^*}),
% \end{align}
% where $\rho \in [0,1]$. Inputs with similarity less than $0.5$ are considered out-of-scope samples, while those with similarity equal to or greater than $0.5$ are regarded as in-scope samples. The final output of the model is:

% \begin{align}
% y_{\text{test}} = 
% \begin{cases}
% f_{\text{base}}(i_{\text{test}}, t_{\text{test}}), & \rho < 0.5 \\
% f_{\text{cfr}}(t_e, y_e, i_{\text{test}}, t_{\text{test}}), & \rho \geq 0.5
% \end{cases}
% \end{align}
% where $f_{\text{base}}$ denotes the base model, and $f_{\text{cfr}}$ denotes the counterfactual model. 

\subsection{Multimodal Scope Classifier}
The multimodal scope classifier in FGVEdit integrates both visual and textual modalities to capture fine-grained similarities between inputs and editing examples.
This integration is crucial because relying solely on textual semantics may not accurately reflect the similarity when $t_e$ and $t_{\text{test}}$ describe different entities related to $i_e$ and $i_{\text{test}}$.

Therefore, our multimodal scope classifier fuses image and text information to comprehensively evaluate the relevance between the query and the editing examples. For images and texts, we first obtain their representations in a unified feature space:

\begin{align}
h^i_e = A_i(E_i(i_e)),&\quad
h^t_e = A_t(E_t(t_e, y_e)),
\\
h^i_{\text{test}} = A_i(E_i(i_{\text{test}})),&\quad
h^t_{\text{test}} = A_t(E_t(t_{\text{test}})),
\end{align}
in which $E_i(\cdot)$ and $E_t(\cdot)$ are encoders for images and texts, respectively, which extract high-level features from the inputs.
The Alignment modules $A_i(\cdot)$ and $A_t(\cdot)$ project the encoded features into a shared multimodal space, ensuring that the image and text representations are compatible for fusion.
To simplify the process, we utilize a pre-trained CLIP model for fine-tuning, which is capable of extracting aligned features from both images and text.

We then compute the image-text fused features:

\begin{align}
z_e &= \text{Fusion}(h^i_e, h^t_e),
\\
z_{\text{test}} &= \text{Fusion}(h^i_{\text{test}}, h^t_{\text{test}}),
\end{align}
in which the $\text{Fusion}(\cdot, \cdot)$ function combines the visual and textual features to capture the cross-modal interactions. This can be implemented using methods like cross-modal attention, where the features from one modality attend to the features of the other, or through simple concatenation followed by a fully connected layer to learn the joint representation.
To simplify the training process, we employ a straightforward dot-product attention mechanism to extract the portions of the image that are relevant to the text.

Finally, the similarity is calculated from the fused features:

\begin{align}
\rho = \text{Sim}(z_e, z_{\text{test}}),
\end{align}
where $\text{Sim}(\cdot, \cdot)$ is a similarity function, such as cosine similarity or a learned distance metric, which quantifies the relevance between the query and the editing example in the fused feature space.
It is important to note that our multimodal scope classifier can accept singel-text input, with the image set to null, ensuring compatibility with singel-modal tasks.


\noindent\textbf{Training}.
We need to train the multimodal range classifier on the MKE dataset to meet our fine-grained visual classification requirements.
The MKE dataset consists of a collection of editing samples denoted as $D_e = \{(i^{k}_e, t^{k}_e, y^{k}_e)\}$. For each editing sample, the dataset provides both in-scope inputs $(i^{k}_{in}, t^{k}_{in})$ and out-of-scope inputs $(i^{k}_{in}, t^{k}_{in})$.

The multimodal scope classifier is treated as a binary classifier, designed to determine whether a given query is related to the editing examples stored in memory.
To train this classifier, we utilize binary cross-entropy loss, which is defined as:

\begin{align}
\rho^{k}_{\text{in}} &= f_{\text{cls}}(i^{k}_{\text{in}}, t^{k}_{\text{in}}, i^{k}_e, t^{k}_e, y^{k}_e),\\
\rho^{k}_{\text{out}} &= f_{\text{cls}}(i^{k}_{\text{out}}, t^{k}_{\text{out}}, i^{k}_e, t^{k}_e, y^{k}_e),
\end{align}
\begin{equation}
\mathcal{L}_{cls} = -\frac{1}{N} \sum_{k=1}^{N} [ \log(\rho^{k}_{\text{in}}) + \log(1 - \rho^{k}_{\text{out}})],
\end{equation}
where $N$ is the total number of training samples.

% The counterfactual model is specifically designed to operate on in-scope inputs $(i^{k}_{in}, t^{k}_{in})$. For each in-scope query, we utilize the corresponding editing samples $(t^{k}_e, y^{k}_e)$ as prompts to guide the model in generating the desired output $y^{k}_{in}$. To train the counterfactual model, we employ a negative log-likelihood loss function:
% \begin{align}
% \mathcal{L}_{cfr} = -\frac{1}{N} \sum_{i=1}^{N} \log p(y^{k}_{in} \mid t^{k}_e, y^{k}_e, i^{k}_{in}, t^{k}_{in}),
% \end{align}
% where $y^{k}_{in}$ is the ground truth output for the $i$-th in-scope query, and $p(y^{k}_{in} \mid t^{k}_e, y^{k}_e, i^{k}_{in}, t^{k}_{in})$ is the predicted probability of the counterfactual model outputting $y^{k}_{in}$ given the in-scope input and the associated editing samples.

==> sec/temp_experiment.tex <==
\section{Experiments and Results}
\subsection{Experimental Setup}
\noindent\textbf{Base MLLMs.}
We utilize BLIP-2 OPT \cite{blip2} and MiniGPT-4 \cite{minigpt} as the base MLLMs for FGVEdit.
%
\textbf{BLIP-2 OPT} is a vision-language model that combines a pre-trained Vision Transformer (ViT) with a lightweight Querying Transformer (Q-Former). It uses a two-stage pre-training strategy: the first stage focuses on learning vision-language representations, while the second emphasizes generative learning, allowing for efficient zero-shot image-to-text generation. 
%
\textbf{MiniGPT-4} integrates a pre-trained ViT with a Q-Former to effectively align visual features with the Vicuna LLM. This architecture enables it to process and generate text based on visual inputs, enhancing its performance on complex vision-language tasks.

\textbf{Baselines.}
Since there are currently no methods specifically designed for FGVEdit, we apply the LLM editing methods to the LLM within MLLMs as baselines for evaluation.
%
\textbf{Fine-tuning} adjusts a pre-trained model’s parameters to incorporate new information. While effective, it is computationally intensive and may unintentionally degrade unrelated behaviors.
%
\textbf{IKE} \cite{ike} is a paradigm that utilizes contextual learning to modify specific factual knowledge in LLMs without altering their parameters. By providing carefully crafted demonstrations as input prompts, IKE guides the model to update its responses to reflect new or corrected information, avoiding the computational costs of fine-tuning.
%
\textbf{SERAC} \cite{serac} stores new facts in an additional memory, and employs a scope classifier to determine whether the input is related to the facts stored in memory. By utilizing a counterfactual model to answer questions related to the new facts while preserving the original model, SERAC enables targeted modifications without accessing the underlying model parameters, thereby enhancing computational efficiency.
%
\textbf{MEND} \cite{mend} leverages an auxiliary neural network to convert fine-tuning gradients into targeted updates, facilitating rapid edits while maintaining performance on unrelated inputs. It serves as a scalable solution for model improvement.

\textbf{Implementation details.}
For SERAC, MEND, and IKE, we utilized the code provided by the EasyEdit\cite{wang2023easyedit} toolkit, while Fine-tuning was implemented using the code from KEBench\cite{kebench}.
Our method was developed based on the SERAC\cite{serac} implementation within the EasyEdit\cite{wang2023easyedit} toolkit. 
Additionally, to comprehensively test our multimodal scope classifier without being constrained by the performance of the counterfactual model, we implemented the FGVEdit-MEND version of our method using MEND as the counterfactual model.

% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table*}[t]
% \renewcommand{\arraystretch}{1.1}
% \centering
% \resizebox{\textwidth}{!}{%
% \tiny
% \begin{tabular}{cccccccc}
% \hline
% Method        & FT-LLM         & FT-Visual      & IKE            & SERAC          & MEND        & FGVEdit           & FGVEdit-MEND      \\ \hline
% \multicolumn{8}{c}{BLIP-2 OPT}                                                                                                    \\ \hline
% Reliability   & \textbf{100.0} & 99.68          & {\ul 99.89}    & 93.08          & 97.00       & 99.13          & 97.40          \\
% T-Locality    & 76.93          & \textbf{100.0} & 48.49          & {\ul 99.90}    & 98.60       & \textbf{100.0} & \textbf{100.0} \\
% T-Generality  & \textbf{99.96} & {\ul 99.21}    & 98.02          & 96.83          & 96.40       & 98.56          & 96.50          \\
% V-Specificity & 24.21          & 16.56          & 20.07          & 31.92          & {\ul 65.85} & 61.60          & \textbf{68.38} \\ \hline
% \multicolumn{8}{c}{MiniGPT-4}                                                                                                     \\ \hline
% Reliability   & 93.39          & 93.39          & \textbf{100.0} & {\ul 99.50}    & 94.85       & {\ul 99.50}    & 97.05          \\
% T-Locality    & 86.26          & \textbf{100.0} & 52.45          & \textbf{100.0} & {\ul 98.58} & \textbf{100.0} & \textbf{100.0} \\
% T-Generality  & 93.35          & 91.87          & \textbf{98.88} & 92.90          & 94.82       & 93.00          & {\ul 96.70}    \\
% V-Specificity & 35.02          & 30.53          & 25.26          & 37.85          & {\ul 67.39} & 57.20          & \textbf{71.98} \\ \hline
% \end{tabular}%

% }
% \caption{Performance comparison of various knowledge editing methods on BLIP-2 OPT and MiniGPT-4. Results are presented as percentages, with the best results in \textbf{bold} and the second-best results \underline{underlined}.}
% \label{tab:results}
% \end{table*}

\begin{table*}[t]
\renewcommand{\arraystretch}{1.1}
\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{ccccccccc}
\hline
Model     & \multicolumn{4}{c}{BLIP-2 OPT}                                    & \multicolumn{4}{c}{MiniGPT-4}                                     \\
Method    & Reliability    & T-Locality     & T-Generality   & V-Specificity  & Reliability    & T-Locality     & T-Generality   & V-Specificity  \\ \hline
FT-LLM    & \textbf{100.0} & 76.93          & \textbf{99.96} & 24.21          & 93.39          & 86.26          & 93.35          & 35.02          \\
FT-Visual & 99.68          & \textbf{100.0} & {\ul 99.21}    & 16.56          & 93.39          & \textbf{100.0} & 91.87          & 30.53          \\
IKE       & {\ul 99.89}    & 48.49          & 98.02          & 20.07          & \textbf{100.0} & 52.45          & \textbf{98.88} & 25.26          \\ \hline
SERAC     & 93.08          & {\ul 99.90}    & 96.83          & 31.92          & {\ul 99.50}    & \textbf{100.0} & 92.90          & 37.85          \\
\rowcolor{gray!20}
FGVEdit      & 99.13          & \textbf{100.0} & 98.56          & 61.60          & {\ul 99.50}    & \textbf{100.0} & 93.00          & 57.20          \\ \hline
MEND      & 97.00          & 98.60          & 96.40          & {\ul 65.85}    & 94.85          & {\ul 98.58}    & 94.82          & {\ul 67.39}    \\
\rowcolor{gray!20}
FGVEdit-MEND & 97.40          & \textbf{100.0} & 96.50          & \textbf{68.38} & 97.05          & \textbf{100.0} & {\ul 96.70}    & \textbf{71.98} \\ \hline
\end{tabular}%

}
\caption{Performance comparison of various knowledge editing methods on BLIP-2 OPT and MiniGPT-4. Results are presented as percentages, with the best results in \textbf{bold} and the second-best results \underline{underlined}.}
\label{tab:results}
\end{table*}

\subsection{Main Results}
Table~\ref{tab:results} presents the results of all editing methods on our benchmark.

\textbf{Reliability}.
Reliability is used to evaluate whether the editing of the target knowledge is successful. As the fundamental objective of knowledge editing, this metric does not pose a significant challenge. Most editing methods achieve nearly perfect scores. Our methods, FGVEdit and FGVEdit-MEND, have achieved consistent improvements over their respective baselines, SERAC and MEND, demonstrating superior reliability.

\textbf{T-Locality}.
T-Locality measures the ability of editing methods to change only the target knowledge in the text space. FT-LLM and IKE perform poorly due to the lack of relevant constraints during the editing process. Only FT-Visual and our FGVEdit achieve a perfect score of 100 on both models. This suggests that our method is highly effective in precisely targeting edits without affecting unrelated information in text space.

\textbf{T-Generality}.
T-Generalization evaluates whether editing methods generalize to similar questions related to the editing target. Although our method is designed for multimodal scenarios, it still outperforms SERAC and MEND on pure text tasks. This demonstrates the versatility of our approach.

\textbf{V-Specificity}.
V-Specificity, an metric specifically designed for multimodal scenarios, necessitates that the model comprehensively considers both image and text in order to delineate fine-grained editing scopes. In contrast, IKE and SERAC, which rely solely on textual information, exhibit significant limitations. Although MEND updates the parameters of both the visual and language modules and performs better than other baselines, there remains room for improvement. Our proposed FGVEdit, through the design of a multimodal classifier that integrates information from both modalities, significantly outperforms SERAC when employing the same counterfactual model. Furthermore, our FGVEdit-MEND consistently demonstrates improvements over MEND, underscoring the advantages of classifier-based editing methods. These results highlight the effectiveness of our approach in addressing complex multimodal editing tasks.

\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \resizebox{\columnwidth}{!}{
   \includegraphics[]{pic/cls.pdf}
}
   \caption{Comparison of classification performance between FGVEdit's multimodal scope classifier and SERAC's classifier on text and image samples.}
   \label{fig:cls}
\end{figure}

\subsection{Analysis of Scope Classifiers}
In the FGVEdit dataset, we developed a multimodal classifier that integrates both image and text information to achieve fine-grained classification of editing scopes. To evaluate the effectiveness of our approach, we compared the performance of scope classifiers in FGVEdit with those in the SERAC dataset. Fig.~\ref{fig:cls} illustrates the classifiers' performance on both text and image samples.

For text samples, both SERAC and FGVEdit classifiers demonstrated high accuracy, indicating that the incorporation of image data in FGVEdit did not compromise the performance of single-modal text classification. This consistency underscores the robustness of our multimodal approach in maintaining strong textual classification capabilities.

Conversely, for image samples, the classifier in SERAC exhibited limited effectiveness, predominantly categorizing nearly all samples as in-scope. This performance shortfall highlights the inherent challenges posed by our benchmark, where fine-grained scenarios are meticulously designed such that both in-scope and out-scope samples' text maintain a certain degree of relevance to the editing targets' text. In this context, the multimodal classifier in FGVEdit achieved significant improvements over SERAC, effectively leveraging the combined textual and visual information to enhance classification accuracy. The ability of FGVEdit's classifier to discern nuanced differences in image data, aided by contextual text information, demonstrates the superior capability of our multimodal approach in handling complex classification tasks.

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
                      & \multicolumn{2}{c}{CLIP-ViT-B/32} & \multicolumn{2}{c}{CLIP-ViT-L/14} \\
                      & Text            & Image           & Text            & Image           \\ \hline
concatenation         & 99.80           & 63.70           & {\ul 99.80}     & 63.80           \\
cross-attention       & {\ul 99.85}     & {\ul 64.45}     & \textbf{99.85}  & {\ul 64.35}     \\
dot-product attention & \textbf{99.95}  & \textbf{64.73}  & {\ul 99.80}     & \textbf{64.85}  \\ \hline
\end{tabular}%
}
\caption{Ablation results of classifier components.}
\label{tab:ablation}
\end{table}

\begin{table*}[t]
\centering
 \resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\hline
\multicolumn{2}{c}{source} & \multicolumn{2}{c}{target} & \multirow{2}{*}{Reliability} & \multirow{2}{*}{T-Locolity} & \multirow{2}{*}{T-Generality} & \multirow{2}{*}{V-Specificity} \\
method     & model         & method      & model        &                              &                             &                               &                                \\ \hline
FGVEdit       & BLIP-2 OPT    & /           & /            & 99.13                        & 100                         & 98.56                         & 64.60                          \\
FGVEdit       & BLIP-2 OPT    & FGVEdit-MEND   & BLIP-2 OPT   & 97.40/97.40                  & 100/100                     & 96.52/96.50                   & 68.35/68.38                    \\
FGVEdit       & BLIP-2 OPT    & FGVEdit        & MiniGPT-4    & 99.50/99.50                  & 100/100                     & 93.11/93.00                   & 57.09/57.20                    \\
FGVEdit       & BLIP-2 OPT    & FGVEdit-MEND   & MiniGPT-4    & 97.10/97.05                  & 100/100                     & 96.82/96.70                   & 72.16/71.98                    \\ \hline
\end{tabular}%
 }
\caption{Transferability of the trained multimodal scope classifier to different editing methods and base models. Results are presented as transfered/retrained, where applicable.}
\label{tab:transfer}
\end{table*}

\begin{table}[]
\centering
\begin{tabular}{ccc}
\hline
               & inference time & model size \\ \hline
classifier     & 36ms           & 0.56G      \\
base           & 121ms          & 9.10G      \\
counterfactual & 85ms           & 4.22G      \\ \hline
\end{tabular}%
\caption{Comparison of inference time and memory usage among the multimodal scope classifier, base model, and counterfactual model on BLIP-2 OPT.}
\label{tab:computational}
\end{table}



\subsection{Ablation Study}
In our multimodal scope classifier, we primarily incorporate a feature extraction module and a feature fusion module. The feature extraction module consists of an encoder and an alignment module, which we implement using CLIP. The feature fusion module is realized through dot-product attention.
To investigate the impact of different components, we tested two versions of CLIP: CLIP-ViT-B/32 and CLIP-ViT-L/14. Additionally, we explored three feature fusion methods: feature concatenation, cross-attention, and dot-product attention. The experimental results are illustrated in Table~\ref{tab:ablation}.

The results indicate that when using both CLIP versions, the performance is remarkably close. This suggests that CLIP-ViT-B/32 is sufficient to extract comprehensive information from the model’s features, demonstrating that our classifier does not require extensive computational resources. Such efficiency is beneficial for practical applications where computational capacity may be limited.
For all fusion methods, we achieved near-perfect accuracy for single-modal text inputs, indicating that these fusion strategies effectively preserve the integrity of textual features in a multimodal setting. This consistency underscores the robustness of our approach in handling textual data.
For image inputs, dot-product attention achieves the best performance while consuming few computational resources.
This superior performance can be attributed to the efficiency of dot-product attention in capturing essential interactions between text and image features without the computational overhead associated with more complex fusion methods like cross-attention. Consequently, dot-product attention serves as an effective and efficient method for feature fusion in our multimodal classifier, particularly when computational resources are limited.


\subsection{Computational Cost Analysis}
To assess the editing overhead introduced by FGVEdit, we compared the inference time and memory usage of the multimodal scope classifier, the base model, and the counterfactual model on BLIP-2 OPT. 
As shown in Table~\ref{tab:computational}, our designed multimodal scope classifier requires significantly less inference time and memory space compared to the base model and counterfactual model. 
These results demonstrate that our classifier introduces minimal computational overhead while playing a decisive role in enhancing editing performance. 
The lightweight nature of the classifier ensures that it does not become a bottleneck in the system, making FGVEdit practical for real-world applications where computational resources may be constrained.

\subsection{}
To further explore the advantages of our multimodal scope classifier, we investigated its transferability across different editing methods and base models.
Specifically, we transferred the scope classifier trained using FGVEdit on BLIP-2 OPT to other settings, such as using MEND as the counterfactual model and employing MiniGPT-4 as the base model.

Table~\ref{tab:transfer} presents our results. Our multimodal scope classifier demonstrated remarkable transferability. In all configurations, the transferred multimodal scope classifier achieved results that were essentially consistent with retrained classifier.
This decoupled design and excellent transferability allow our method to be rapidly deployed on new MLLMs. 
